Leaping Through Time with Gradient-based Adaptation for Recommendation

Modern recommender systems are required to adapt to the change in user preferences and item popularity. Such a problem is known as the temporal dynamics problem, and it is one of the main challenges in recommender system modeling. Different from the popular recurrent modeling approach, we propose a new solution named LeapRec to the temporal dynamic problem by using trajectory-based meta-learning to model time dependencies. LeapRec characterizes temporal dynamics by two complement components named global time leap (GTL) and ordered time leap (OTL). By design, GTL learns long-term patterns by finding the shortest learning path across unordered temporal data. Cooperatively, OTL learns short-term patterns by considering the sequential nature of the temporal data. Our experimental results show that LeapRec consistently outperforms the state-of-the-art methods on several datasets and recommendation metrics. Furthermore, we provide an empirical study of the interaction between GTL and OTL, showing the effects of long- and short-term modeling.

==> table/exp-full-test.tex <==
\newcommand{\static}{{\scriptsize \faStop}}
\newcommand{\sequence}{{\scriptsize \faForward}}
\newcommand{\temporal}{{\scriptsize \faClock[regular]}}
\newcommand{\stream}{{\scriptsize \faPlayCircle}}
\begin{table*}[htbp]
    \centering
    \small
      \begin{adjustbox}{max width=\textwidth}
      \begin{tabular}{lcccc cccccccc}
      \toprule
      \multirow{2}[4]{*}{Model} & \multicolumn{4}{c}{Amazon} & \multicolumn{4}{c}{Goodreads} & \multicolumn{4}{c}{Yelp} \\
    
      \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}      & \scriptsize{HR@1}  & \scriptsize{HR@5}  & \scriptsize{NDCG@5}  & \scriptsize{MRR@100} & \scriptsize{HR@1}  & \scriptsize{HR@5}  & \scriptsize{NDCG@5}  & \scriptsize{MRR@100} & \scriptsize{HR@1}  & \scriptsize{HR@5}  & \scriptsize{NDCG@5}  & \scriptsize{MRR@100} \\
      \midrule
    \static{} BPR & .00047 & .00178 & .00112 & .00166 & .00309 & .01280 & .00791 & .01072 & .00261 & .01109 & .00680 & .00947 \\

    \sequence{} NARM & .00049 & .00222 & .00137 & .00191 & \underline{.00487} & \underline{.01871} & \underline{.01173} & \underline{.01515} & .00260 & .01173 & .00700 & .00961 \\
    \sequence{} SASRec & .00063 & .00216 & .00139 & .00185 & .00460 & .01713 & .01075 & .01397 & \underline{.00342} & .01368 & .00851 & .01143 \\
    \temporal{} TiSASRec & \underline{.00076} & \underline{.00228} & \underline{.00151} & \underline{.00202} & \textbf{.00499} & .01840 & .01167 & .01462 & .00341 & \underline{.01404} & \underline{.00868} & \underline{.01164} \\

    % \textbf{LeapRec-MF} \\
    \rule{0pt}{2ex}    
    \textbf{LeapRec} & \textbf{.00123} & \textbf{.00528} & \textbf{.00324} & \textbf{.00413} & .00471 & \textbf{.02205} & \textbf{.01326} & \textbf{.01724} & \textbf{.00446} & \textbf{.01755} & \textbf{.01092} & \textbf{.01443} \\      \bottomrule
      \end{tabular}%
    \end{adjustbox}
      
    \caption{Performance comparison of different models evaluating by ranking \emph{all unseen items}. The best performances are highlighted in bold. The second best performances are underlined. The symbols \static, \sequence, and \temporal\ denote static, sequential, and temporal models, respectively.}     
    \label{tab:exp-full-test}%
  \end{table*}%


==> table/exp-gnn.tex <==
\begin{table*}[t]
  \centering
  \small
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}[4]{*}{Model} & \multicolumn{3}{c}{Amazon} & \multicolumn{3}{c}{Goodreads} & \multicolumn{3}{c}{Yelp} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
     & $L=1$ & $L=2$ & $L=3$ & $L=1$ & $L=2$ & $L=3$ & $L=1$ & $L=2$ & $L=3$ \\
    \midrule
    GCN & 0.143 & 0.156 & 0.161 & 0.345 & 0.353 & 0.360 & 0.457 & 0.486 & 0.504 \\
    \model-GCN & 0.224 & \textbf{0.239} & 0.229 & \textbf{0.403} & 0.394 & 0.380 & 0.524 & \textbf{0.530} & 0.533 \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
    \emph{Improvement} & 56.76\% & 52.93\% & 42.47\% & 16.87\% & 11.79\% & 5.72\% & 14.48\% & 9.05\% & 5.77\% \\

    \midrule
    NGCF & 0.142 & 0.149 & 0.152 & 0.349 & 0.361 & 0.350 & 0.470 & 0.469 & 0.473 \\
    \model-NGCF & 0.164 & 0.224 & 0.234 & 0.369 & 0.384 & 0.385 & 0.483 & 0.506 & 0.520 \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
    
    \emph{Improvement} & 15.24\% & 50.09\% & 53.57\% & 5.93\% & 6.36\% & 9.90\% & 2.74\% & 7.90\% & 10.00\% \\
    \midrule
    LightGCN & 0.155 & 0.168 & 0.173 & 0.365 & 0.370 & 0.374 & 0.487 & 0.502 & 0.511 \\
    \model-LightGCN & 0.165 & 0.194 & 0.212 & 0.363 & 0.369 & 0.367 & 0.485 & 0.500 & 0.497 \\
    % \hline
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
    \emph{Improvement} & 5.96\% & 15.46\% & 22.70\% & -0.62\% & -0.30\% & -1.78\% & -0.43\% & -0.37\% & -2.64\% \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
    \caption{Performance comparison (NDCG@5) between GNNs without and with \model{} with different numbers of layers $L$}
  \label{tab:exp-gnn}%
\end{table*}%


==> table/exp-leap-base.tex <==

\begin{table}[tb]
    \centering
    \small
      \begin{tabular}{lccc}
      \toprule
      Model & Amazon & Goodreads & Yelp \\
      \midrule
BPR & 0.1629 & 0.3662 & 0.4823 \\
LeapRec-BPR & 0.1506 & 0.3867 & 0.5034 \\
\cmidrule(lr){1-4}
\emph{Improvement} & -7.51\% & 5.60\% & 4.38\% \\
\midrule
NCF & 0.1506 & 0.3630 & 0.4857 \\
LeapRec-NCF & 0.1734 & 0.4077 & 0.5071 \\
\cmidrule(lr){1-4}
\emph{Improvement} & 15.14\% & 12.3\% & 4.40\% \\
\bottomrule
      \end{tabular}%
    \caption{Performance (NDCG@5) of BPR and NCF without and with LeapRec}
    \label{tab:exp-leap-base}%
  \end{table}%

